Gauge-mediated supersymmetry breaking with generalized messenger sector at LHC

We consider the generalized gauge mediated supersymmetry breaking (GMSB) models with the messenger fields which do not form the complete multiplets of SU(5) GUT symmetry. Such a situation may happen in the anomalous U(1) GUT scenario because the mass spectrum of the superheavy particle does not respect SU(5) GUT symmetry, although the success of the gauge coupling unification can be explained. In this paper, we assume that one pair of the messenger fields gives the dominant contribution, and the LHC signature for the two possible messengers, X + \bar{X} and Q + \bar{Q}, are examined. We investigate the possibility to measure the deviation from the usual GUT relation of the gaugino masses which is one of the most important features of these scenarios.

==> feature.tex <==
%To obtain the meaningful information from the LHC measurement,
%we must study the signal before proceeding to the detailed measurement
%of mass spectrum.
%Without understanding the feature of the spectrum, we cannot make
%a plan to analyze them.

First of all, we figure out several features for three cases in
$X + \bar{X}$ messenger scenario and  one case in $Q + \bar{Q}$
messenger scenario.
\begin{enumerate}
\item $m_{\tilde W} : m_{\tilde g} \sim 1:2$ in both scenarios.
      As the result, the ratio $m_{\tilde W}/m_{\tilde q}$ becomes
      larger than in the usual scenario with the GUT
      relation. Roughly speaking, the hierarchy between colored sparticles
      and wino masses becomes milder.
\item $m_{\tilde B} \sim m_{\tilde W}$ in the $X+\bar X$ messenger scenario.
      In most of the interesting parameter region, the decay mode 
      $\chi_2^0\rightarrow Z\chi_1^0$ is closed, and therefore,
      the branching ratios of leptonic decay modes of $\chi_2^0$
      become comparatively large. The leptonic modes are important
      in obtaining meaningful information from the data in the LHC.
\item $m_{\tilde B} \ll m_{\tilde W}$ in the $Q+\bar Q$ messengner scenario.
\end{enumerate}
In the followings, we study how to catch these features from the LHC signals.

In region 3 of $X + \bar{X}$ messenger scenario, very peculiar signal
is expected because the NLSP becomes the right-handed stau.
The momentum and velocity of stau which goes out the detector can be
measured, and therefore, we can know the masses of various SUSY particles by
using the invariant mass technique and the above features can be tested.
%calculate the invariant masses of various SUSY particles.  by means of muon system.
%Since the required analysis in this case is quite different from
%he other scenarios, 
We discuss the mass measurements for this case
%separately 
in subsection \ref{sec:x3}.

\begin{figure}
 \begin{center}
   \includegraphics[scale=1.0]{gr_tree.pdf}
 \caption{Decay chains which we use for the analysis in this paper.
 $\tilde{\chi}_2^0$ decays to $\tilde{\chi}_1^0$ via the off-shell
 slepton in the case 1. In the case 2, $\tilde{\chi}_2^0$ decays to on-shell
 slepton and we label the leptons which come from the decay of
 $\tilde{\chi}_2^0$ and $\tilde{l}_R$ as $l_n$ and $l_f$, respectively.}
 \label{fig:tree}    
 \end{center}
\end{figure}

Here, we concentrate on discussing the cases 1 and 2 of
$X + \bar{X}$ messenger scenario and $Q + \bar{Q}$ messenger scenario.
Since we are interested in the measurement related to the masses of
the bino and wino, we make use of the characteristic decay modes
of these particles.
As noted in the comment of feature 2, 
for $X+\bar X$ messenger scenario, %as can be seen in Table \ref{tab:parmx} and \ref{tab:parmq},
%we can use 
the leptonic decay of wino-like neutralino $\tilde{\chi}_2^0$
to the lightest bino-like neutralino $\tilde{\chi}_1^0$
through on-shell or off-shell slepton $\tilde{l}_R$ is useful,
which are illustrated in Figure \ref{fig:tree}.
Note that since the higgsino-like neutralinos prefer to decay to tau-lepton rather
than electron and muon, we can avoid the gaugino-higgsino ambiguity
in the measurement of gaugino-like neutralino mass in this leptonic decay to
the electrons and muons.

\begin{figure}
 \begin{center}
  \begin{tabular}{ccc}
   \includegraphics[scale=0.75]{gr_x1_1.pdf} &
   \includegraphics[scale=0.75]{gr_x2_1.pdf} &
   \includegraphics[scale=0.75]{gr_q_7.pdf}   
  \end{tabular}
 \caption{Dilepton invariant mass $m_{ll}$ distributions for
 $10\,\mathrm{fb}^{-1}$ of each model points.
  The bins illustrated by the dotted line represents the similar
  distribution using the opposite-sign and different flavor
  dileptons ($e^+\,\mu^- + \mu^+\,e^-$).}
 \label{fig:mll}     
 \end{center}
\end{figure}

First, we consider the invariant mass of a pair of leptons
coming from the decay of $\tilde{\chi}_2^0$.
As can be seen from Table \ref{tab:parmx}, in the $X+\bar X$ messenger
scenario, a large number of
$\tilde{\chi}_2^0$ is expected to be produced via the decay of
left-handed squark $\tilde{q}_L$.
We use a dilepton with opposite-sign and same-flavor
($e^+\,e^- + \mu^+\,\mu^-$) for making the invariant mass
and the distribution shown in Figure \ref{fig:mll} is obtained.
In this figure, the background is estimated by taking the similar
invariant mass of dilepton with opposite-sign and different-flavor
($e^+\,\mu^- + \mu^+\,e^-$).
Here, in order to reduce the SM background, we impose following event
cuts by using the transverse momenta $p_T$
\begin{itemize}
 \item $p_{T}^{(1)} > 100\,\mathrm{GeV}$ and
       $p_{T}^{(2,3,4)} > 50\,\mathrm{GeV}$
 \item $M_{\text{eff}} \equiv p_T^{(1)} + p_T^{(2)} + p_T^{(3)} +
       p_T^{(4)} + E_T^{\text{miss}} > 400\,\mathrm{GeV}$
 \item $E_T^{\text{miss}} > \max\{100\,\mathrm{GeV},0.2M_{\text{eff}}\}$
 \item Two isolated leptons with $p_T^e > 20\,\mathrm{GeV}$ and
       $p_T^{\mu} > 5\,\mathrm{GeV}$       
\end{itemize}
where $p_T^{(i)}$ means the $i$-th largest $p_T$ of the jet in
each event and
$E_T^{\text{miss}} = \sqrt{(p_x^{\text{miss}})^2 + (p_y^{\text{miss}})^2}$.
Since the SM background is reduced successfully after
these cut, we generate only events of sparticle production for
our simulation.

We can see the rather small maximum value of invariant mass
 for both cases of the  $X + \bar{X}$ scenario
in Figure \ref{fig:mll}, which is caused by the feature 2, namely, 
$m_{\tilde B}\sim m_{\tilde W}$.
%the interpretation of this is not straightforward.
%The troublesome point is that the meaning of kinematical endpoint is
%different between case 1 and case 2.
%Since the decay of $\tilde{\chi}_2^0$ is three body decay in case 1,
Actually, the maximum value of invariant mass allowed by
kinematics is given as
\begin{equation}
 \label{eq:x1ll}
 m_{ll}^{\max}[\text{Case 1}] = m_{\tilde{\chi}_2^0} - m_{\tilde{\chi}_1^0}
\end{equation}
in region 1, and 
%On the other hand, the decay through on-shell slepton leads to
%the different maximum value of the dilepton invariant mass
\begin{equation}
 (m_{ll}^{\max}[\text{Case 2}])^2 = m_{\tilde{\chi}_2^0}^2
  \left(1 - \frac{m_{\tilde{l}_R}^2}{m_{\tilde{\chi}_2^0}^2}\right)
  \left(1 - \frac{m_{\tilde{\chi}_1^0}^2}{m_{\tilde{l}_R}^2}\right)  
\end{equation}
in region 2, which result in rather small maximum value of the invariant
mass calculated as
%In each cases, the theoretical values predicted from the mass spectra
%given in Table \ref{tab:parmx} are
\begin{equation}
 m_{ll}^{\max}[\text{Case 1}] = 44\,\mathrm{GeV},\qquad
 m_{ll}^{\max}[\text{Case 2}] = 47\,\mathrm{GeV}.
\end{equation}
Unfortunately, the smallness of $m_{ll}^{\max}$ does not always mean the 
smallness of the mass splitting between the bino and wino.
%the small maximum value of the invariant mass does not
%mean $m_{\tilde B}\sim m_{\tilde W}$. 
For the case 2, if one of the relations
$m_{\tilde B}\sim m_{\tilde l}$ and $m_{\tilde l}\sim m_{\tilde W}$ is
satisfied, the maximum value of the invariant mass becomes small.
%If we know that the obtained distribution corresponds to that of case 1,
%we can see the mass difference of bino and wino directly.
%However we do not have any reliable information to judge the spectra
%to be case 1 or case 2 yet.
%So
\begin{figure}
 \begin{center}
  \includegraphics[scale=0.75]{gr_ptl_x1.pdf}
  \includegraphics[scale=0.75]{gr_ptl_x2.pdf}
  \includegraphics[scale=0.75]{gr_ptl_q.pdf}  
 \end{center}
 \caption{$p_T$ distributions of leptons emitted from sparticle decays.
 Each graphs corresponds to $1\,\mathrm{fb}^{-1}$ for the case 1 of
 $X + \bar{X}$ scenario (left),
 $1\,\mathrm{fb}^{-1}$ for the case 2 of $X + \bar{X}$ scenario (center)
 and $10\,\mathrm{fb}^{-1}$ for $Q + \bar{Q}$ scenario (right).} 
 \label{fig:ptl} 
\end{figure}

To check that the mass difference between $\tilde{\chi}_1^0$ and
$\tilde{\chi}_2^0$ is small in $X + \bar{X}$ scenario,
we examine the $p_T$ distribution of leptons which come from the
decay shown in Figure \ref{fig:tree}.
Since the magnitute of $p_T$ of produced particles is strongly dependent 
on the volume of the phase space in the decay, this can be a good 
signal to distinguish these scenarios. 
We can see from Figure \ref{fig:ptl} that these leptons
have relatively small $p_T$ in the $X+\bar X$ scenario and
large $p_T$ in the $Q+\bar Q$ scenario.
These are caused by $m_{\tilde B}\sim m_{\tilde W}$ in the $X+\bar X$ scenario
and $m_{\tilde B}\ll m_{\tilde W}$ in the $Q+\bar Q$ scenario.


%This fact means that $m_{\tilde{\chi}_2^0} - m_{\tilde{\chi}_1^0}$ is
%small compared with $m_{\tilde{\chi}_{1,2}^0}$.
%On the other hand, since the mass difference is large in the $Q+\bar Q$ scenario, 
%$p_T$ of leptons becomes comparatively large as shown in Fig. ??.
%Note that the feature 1 is also important to obtain such a small $p_T$
%leptons.


%To obtain the more solid evidence of this scenario, we have to
%carry out the detailed analysis.
%Since we cannot distinguish case 1 and case 2 at this stage,
%we must solve this ambiguity to measure the masses of neutralinos.
%This topic is discussed in section \ref{sec:x12}.

%On the other hand, we cannot see the dilepton signal other than
%the one which comes from the decay of $Z$ boson in $Q + \bar{Q}$
%scenario.
%This is because the decay of $\tilde{\chi}_2^0$ to $Z$ boson and the
%lightest Higgs is dominant in this scenario.
%So we have to correct more luminosity to see the dilepton signal.
%The detailed analysis is given in section \ref{sec:q}, and
%our goal is to show that there is a large hierarchy between
%bino and wino masses in this scenario.
In the following subsections, we examine how to fix the masses
of $\chi_1^0$ and $\chi_2^0$. Once we know $m_{\chi_2^0}\sim 500$ GeV,
we can check the feature 1 by estimating the colored sparticle masses
by $m_{T2}$ method \cite{Lester:1999tx,Barr:2003rg,Barr:2009wu}.
%Another promising way to derive the information of mass spectra
%in low luminocity is $m_{T2}$ measurement.
When we consider the production process of sparticle pair which decay
into a pair of the NLSPs and a pair of the SM particles, 
we can make use of the $m_{T2}$ variable defined by
\begin{equation}
 \label{eq:mt2}
 m_{T2}(M_{\text{test}}) \equiv \min_{\bm{p}_T^{\text{miss}}
 = \sum_i\bm{p}_T^{\chi(i)}}
 \left[\max
  \left\{m_T(\overrightarrow{p}_T^{\text{vis}(1)},
   \overrightarrow{p}_T^{\chi(1)}),
   m_T(\overrightarrow{p}_T^{\text{vis}(2)},
   \overrightarrow{p}_T^{\chi(2)})\right\}\right].
\end{equation}
%where with the knowledge of the emitted observable
%particles whose total momenta are $p_{\mu}^{\text{vis}(1)}$ and
%$p_{\mu}^{\text{vis}(2)}$.
Here $\overrightarrow{p}_T$ is a $(2 + 1)$-dimensional
vector, $\overrightarrow{p}_T \equiv (E_T,\bm{p}_T)$, and 
$p_T^{\text{vis}(i)}$ is the transverse momentum
for the emitted observed particles.
$m_T$ is given by
\begin{equation}
 m_T^2(\overrightarrow{p}_T^{\text{vis}},\overrightarrow{p}_T^{\chi})
  \equiv (\overrightarrow{p}_T^{\text{vis}} + \overrightarrow{p}_T^{\chi})^2
  = m_{\text{vis}}^2 + M_{\text{test}}^2
  + 2(E_T^{\text{vis}}\cdot E_T^{\chi}
  - \bm{p}_T^{\text{vis}} \cdot \bm{p}_T^{\chi})
\end{equation}
where $E_T^{\text{vis}} \equiv
\sqrt{m_{\text{vis}}^2 + |\bm{p}^{\text{vis}}_T|^2}$
and $E_T^{\chi} \equiv \sqrt{M_{\text{test}}^2 + |\bm{p}^{\chi}_T|^2}$.

Now we consider the process
$p\,p \to \tilde{q}\,\tilde{q} \to
\tilde{\chi}_1^0\,q\,\tilde{\chi}_1^0\,q$.
In this process, $m_{\text{vis}}^{(1)} \simeq m_{\text{vis}}^{(2)}
\simeq 0$ and the maximum value of $m_{T2}$ is given by
\begin{equation}
 \label{eq:x1mt2}
 m_{T2}^{\max}(M_{\text{test}}) =
  \frac{m_{\tilde{q}}^2 - m_{\tilde{\chi}_1^0}^2}{2m_{\tilde{q}}}
  + \sqrt{
  \left(
   \frac{m_{\tilde{q}}^2 - m_{\tilde{\chi}_1^0}^2}{2m_{\tilde{q}}}
  \right)^2 + M_{\text{test}}^2}
\end{equation}
as a function of the test mass $M_{\text{test}}$.
Therefore, we can obtain the rough value of the colored sparticle masses
by this analysis.

For the analysis of $m_{T2}$, we use the event cuts
\begin{itemize}
 \item Two jets with $p_T > 100\,\mathrm{GeV}$
 \item $M_{\text{eff}} \equiv p_T^{(1)} + p_T^{(2)} + E_T^{\text{miss}}
       > 400\,\mathrm{GeV}$
 \item $E_T^{\text{miss}} > \max\{100\,\mathrm{GeV},0.2M_{\text{eff}}\}$
 \item No lepton
\end{itemize}
instead of the usual cut for the SM events introduced above.
Since we can induce the information by measuring the distribution for
some fixed $M_{\text{test}}$, we set $M_{\text{test}} = 0$ for
our analysis. Then $m_{T2}^{\max}$ is given as
\begin{equation}
 \label{eq:mt20}
 m_{T2}^{\max}(0) =
  \frac{m_{\tilde{q}}^2 - m_{\tilde{\chi}_1^0}^2}{m_{\tilde{q}}}
\end{equation}
for the process of squark pair production.
The distribution of this quantity is shown in Figure \ref{fig:mt2}.
If the mass of the LSP is very small compared with the mass of
squark, we can interpret $m_{T2}^{\max}(0)$ as the mass scale of
squark.
In fact, this is the case for $Q + \bar{Q}$ messenger scenario.
However, the mass hierarchy of sparticles is small in $X + \bar{X}$
messenger scenario and the effect of $m_{\tilde{\chi}_1^0}$ is
non-negligible.
The theoretical values of $m_{T2}^{\max}(0)$
% for $m_{\tilde{q}} = 1000\,\mathrm{GeV}$ is
are
\begin{equation}
 \label{eq:x1chi}
 m_{T2}^{\max}(0)[\text{Case 1}] = 844\,\mathrm{GeV},\qquad
 m_{T2}^{\max}(0)[\text{Case 2}] = 904\,\mathrm{GeV}.  
\end{equation}
Here we approximate $m_{\tilde q}=1000$ GeV for the case 1 and
$m_{\tilde q}=1100$ GeV for the case 2.
By this analysis, we can obtain the evidence of milder hierarchy 
between the masses of $\chi_2^0$ and colored sparticle
if we know $m_{\tilde{\chi}_2^0} \simeq 500\,\mathrm{GeV}$.
\begin{figure}
 \begin{center}
  \begin{tabular}{ccc}
   \includegraphics[scale=0.75]{gr_x1_4.pdf} &
   \includegraphics[scale=0.75]{gr_x2_4.pdf} &
   \includegraphics[scale=0.75]{gr_q_6.pdf}
  \end{tabular}
 \caption{$m_{T2}$ distributions for $M_{\text{test}} = 0$.}
 \label{fig:mt2}    
 \end{center}
\end{figure}

